Exploring the AGN-Merger Connection in Arp 245 I: Nuclear Star Formation and Gas Outflow in NGC 2992

Galaxy mergers are central to our understanding of galaxy formation, especially within the context of hierarchical models. Besides having a large impact on the star formation history, mergers are also able to influence gas motions at the centre of galaxies and trigger an Active Galactic Nucleus (AGN). In this paper, we present a case study of the Seyfert galaxy NGC 2992, which together with NGC 2993 forms the early-stage merger system Arp 245. Using Gemini Multi-Object Spectrograph (GMOS) integral field unit (IFU) data from the inner 1.1 kpc of the galaxy we were able to spatially resolve the stellar populations, the ionisation mechanism and kinematics of ionised gas. From full spectral synthesis, we found that the stellar population is primarily composed by old metal-rich stars (t $\geq$ 1.4 Gyr, $Z \geq 2.0$\zsun), with a contribution of at most 30 per cent of the light from a young and metal-poor population (t $\leq$ 100 Myr, $Z \leq 1.0$\zsun). We detect \halpha and \hbeta emission from the Broad Line Region (BLR) with a Full Width at Half Maximum (FWHM) of $\sim$ 2000\kms. The Narrow Line Region (NLR) kinematics presents two main components: one from gas orbiting the galaxy disk and a blueshifted (velocity $\approx$ -200\kms) outflow, possibly correlated with the radio emission, with mass outflow rate of $\sim$ 2 M$_{\odot}$ yr$^{-1}$ and a kinematic power of $\sim$ 2 $\times 10^{40}$ erg s$^{-1}$ (\Eout/\Lbol $\approx$ 0.2 per cent). We also show even though the main ionisation mechanism is the AGN radiation, ionisation by young stars and shocks may also contribute to the emission line ratios presented in the innermost region of the galaxy.

==> broad_fit.tex <==
\begin{table*}
\begin{center}
\caption{Fit parameters for the broad H lines}
\begin{tabular}{lcccc}
\hline
\hline
Component & H~$\alpha$ & H~$\beta$ & $\sigma$ & $v_0$ \\
 & $10^{-13}\,\,{\rm erg\,s^{-1}\,cm^{-2}}$ & $10^{-13}\,\,{\rm erg\,s^{-1}\,cm^{-2}}$ & $\mathrm{km\,s^{-1}}$ & $\mathrm{km\,s^{-1}}$ \\
\hline
Component 0 & 8.3 & 0.4 & 428 & -1999 \\
Component 1 & 428.8 & 20.3 & 854 & 10 \\
Component 2 & 10.1 & 0.5 & 435 & 1954 \\
\hline
\end{tabular}
\end{center}
\end{table*}

